SANA 1.5: Efficient Scaling of Training-Time and Inference-Time Compute in Linear Diffusion Transformer

This paper presents SANA-1.5, a linear Diffusion Transformer for efficient scaling in text-to-image generation. Building upon SANA-1.0, we introduce three key innovations: (1) Efficient Training Scaling: A depth-growth paradigm that enables scaling from 1.6B to 4.8B parameters with significantly reduced computational resources, combined with a memory-efficient 8-bit optimizer. (2) Model Depth Pruning: A block importance analysis technique for efficient model compression to arbitrary sizes with minimal quality loss. (3) Inference-time Scaling: A repeated sampling strategy that trades computation for model capacity, enabling smaller models to match larger model quality at inference time. Through these strategies, SANA-1.5 achieves a text-image alignment score of 0.81 on GenEval, which can be further improved to 0.96 through inference scaling with VILA-Judge, establishing a new SoTA on GenEval benchmark. These innovations enable efficient model scaling across different compute budgets while maintaining high quality, making high-quality image generation more accessible. Our code and pre-trained models are released.

==> figures_latex/growth_strategy_loss_curve.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/8_growth_strategy.png}
    \vspace{-0.3cm}
    \caption{\textbf{Comparison of different initialization strategies.} Partial Preservation Init shows stable training behavior while Cyclic and Block Replication strategies suffer from training instability (NaN losses).}
    \label{fig:init_strategies_loss_curve}
\end{figure}

==> figures_latex/qualitative_vis_prune.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/viz-prune.pdf}
    \caption{Qualitative visualization of the generated images from the pruned model. Pruning low-importance score blocks gradually impairs the high-frequency details of the generation. \enze{should we exchange the order of Fig 3 and 4?}}
    \label{fig:viz-prune}
\end{figure*}


==> sections/0_abstract.tex <==
\begin{abstract}
    This paper presents \model{}-1.5, a linear Diffusion Transformer for efficient scaling in text-to-image generation. Building upon \model{}-1.0, we introduce three key innovations: (1) Efficient Training Scaling: A depth-growth paradigm that enables scaling from 1.6B to 4.8B parameters with significantly reduced computational resources, combined with a memory-efficient 8-bit optimizer. 
    (2) Model Depth Pruning: A block importance analysis technique for efficient model compression to arbitrary sizes with minimal quality loss. 
    (3) Inference-time Scaling: A repeated sampling strategy that trades computation for model capacity, enabling smaller models to match larger model quality at inference time.
    Through these strategies, \model{}-1.5 achieves a text-image alignment score of 0.72 on GenEval, which can be further improved to 0.80 through inference scaling, establishing a new SoTA on GenEval benchmark.
    These innovations enable efficient model scaling across different compute budgets while maintaining high quality, making high-quality image generation more accessible. Our code and pre-trained models will be released.
\end{abstract}


==> tables/dpg_hard.tex <==
\begin{table*}[t]
    \centering
    \caption{Quantitative results from DPG-bench Hard, our internal benchmark powered by GPT4-o. \enze{placeholder } \ligeng{add vila template to highlight opensource model and commercial models}}
    \label{tab:dpg_bench}
    \scalebox{0.8}{
    \begin{tabular}{lccccccc}
    \toprule
    \textbf{Method} & \textbf{Overall} & \textbf{Entity} & \textbf{Global} & \textbf{Relation} & \textbf{Position} & \textbf{Count} & \textbf{Text} \\
    \midrule
    SD3-Medium~\cite{sd3} & 53.13 & 61.57 & 73.27 & 49.25 & 50.00 & 51.82 & 18.10 \\
    PixArt-Sigma~\cite{chen2024pixart} & 62.89 & 76.85 & 83.46 & 59.33 & 73.98 & 59.71 & 11.97 \\
    Midjourney v6.0 & 64.63 & 76.86 & 82.86 & 61.29 & 78.12 & 65.36 & 14.30 \\
    DALLE 3~\cite{Dalle-3} & 67.71 & 79.11 & 85.94 & 64.48 & 57.35 & 62.82 & 28.84 \\
    Flux-pro~\cite{FLUX} & 78.69 & 88.68 & 90.62 & 75.15 & 70.58 & 81.13 & 69.47 \\
    Ideogram-1.0 & 79.75 & 89.32 & 90.21 & 78.73 & 78.12 & 65.36 & 47.53 \\
    Ideogram-2.0 & 80.12 & 89.81 & 91.04 & 79.93 & 83.33 & 83.72 & 75.32 \\
    Playground v3~\cite{liu2024playground} & 88.62 & 94.45 & 93.64 & 86.47 & 87.21 & 84.30 & 82.09 \\
    \midrule
    \textbf{SANA-4.8B} & 77.37 & 88.36 & 90.00 & 73.10 & 62.50 & 62.50 & 33.63 \\
    \textbf{SANA-4.8B Inference Scaling} & 78.21 & 90.61 & 91.04 & 73.93 & 100 & 77.77 & 39.20 \\
    \bottomrule
    \end{tabular}
    }
\end{table*}
